Toward Textual Transform Coding

Inspired by recent work on compression with and for young humans, the success of transform-based approaches to information processing, and the rise of powerful language-based AI, we propose \emph{textual transform coding}. It shares some of its key properties with traditional transform-based coding underlying much of our current multimedia compression technologies. It can form the basis for compression at bit rates until recently considered uselessly low, and for boosting human satisfaction from reconstructions at more traditional bit rates.

==> app.tex <==
\section{Omitted Proofs}
\begin{lem}[Lemma~\ref{lem:increasing-entropy} in the main text]
The function $k\mapsto H(X|Y[k])$ is monotone-increasing.
\end{lem}
\begin{proof}
Take $0\leq i\leq j\leq n.$ We wish to prove that $H(X|Y[i])\leq  H(X|Y[j]).$ Since $X\to Y[i] \to Y[j]$ forms a Markov chain, by the data processing inequality we have $I(X;Y[i])\geq I(X;Y[j]).$ But since $H(X) = n,$ this implies $H(X|Y[i])\leq H(X|Y[j]),$ as desired.
\end{proof}


\begin{lem}\label{lem:binom-stirling}
For $u \in \{0,1,\dots,n\}$ and $n\geq 1$, we have
\[
\frac{1}{n}\log \binom{n}{u} \geq h(u/n) - \frac{1}{2n}\log (\max\{2\pi u(n-u)/n,1\}) - \frac{\log e}{6n\max\{\min\{u, (n-u)\}, 1\}}.
\]
\end{lem}
\begin{proof}
The lemma follows from Stirling's approximation 
\[
 m\log m - m\log e + \frac{1}{2}\log(2\pi m) + \frac{1}{12 m+1} \log e\leq \log m! \leq m\log m - m\log e + \frac{1}{2}\log(2\pi m) + \frac{1}{12 m} \log e
\]
applied to each term in the expression $\log\binom{n}{u} = \log n! - \log (u)! - \log (n-u)!,$ and the simple inequality
\[
\frac{1}{12 n - 1} - \frac{1}{12u} - \frac{1}{12(n-u)} \geq \frac{-1}{6n\min\{u, n-u\}}.
\]
We skip the details of the computation. The maxima with 1 are to fix the cases where $u = 0$ or $n.$
\end{proof}


